METR: Image Watermarking with Large Number of Unique Messages

Improvements in diffusion models have boosted the quality of image generation, which has led researchers, companies, and creators to focus on improving watermarking algorithms. This provision would make it possible to clearly identify the creators of generative art. The main challenges that modern watermarking algorithms face have to do with their ability to withstand attacks and encrypt many unique messages, such as user IDs. In this paper, we present METR: Message Enhanced Tree-Ring, which is an approach that aims to address these challenges. METR is built on the Tree-Ring watermarking algorithm, a technique that makes it possible to encode multiple distinct messages without compromising attack resilience or image quality. This ensures the suitability of this watermarking algorithm for any Diffusion Model. In order to surpass the limitations on the quantity of encoded messages, we propose METR++, an enhanced version of METR. This approach, while limited to the Latent Diffusion Model architecture, is designed to inject a virtually unlimited number of unique messages. We demonstrate its robustness to attacks and ability to encrypt many unique messages while preserving image quality, which makes METR and METR++ hold great potential for practical applications in real-world settings. Our code is available at https://github.com/deepvk/metr

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> figures/metr_different_m.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[htp]{0.2\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/messages_same_noise/no_watermark.png}
        \subcaption{no WM}
        % \vspace{0.1\textwidth}
    \end{subfigure}
    \begin{subfigure}[htp]{0.2\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/messages_same_noise/ones.png}
        \subcaption{$m=1111111111$}
        % \vspace{0.1\textwidth}
    \end{subfigure}
    \begin{subfigure}[htp]{0.2\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/messages_same_noise/zeroes.png}
        \subcaption{$m=0000000000$}
    \end{subfigure}
    \begin{subfigure}[htp]{0.2\textwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{images/messages_same_noise/alternating.png}
        \subcaption{$m=1010101010$}
    \end{subfigure}
    \vspace{0.025\textwidth}
\caption{Original image and the corresponding one with a \METR watermark, generated from the same noise with different messages encrypted with a fixed radius $r$ and message scale $S=100$.}
\vspace{0.035\textwidth}
\label{fig:different_m}
\end{figure*}

==> figures/radius_plot_metr_table.tex <==
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{images/graphs/fid_gen_r.png}
%     \caption{\METR evaluation on image quality with different radii}
% \vspace{0.02\textwidth}
% \label{fig:fid_gen_r}
% \end{figure}

% \begin{table}[h]
% \centering
% \caption{
%     Detection metrics for \TR and \METR. Note that \METR is almost as resilient to the attacks as \TR watermark.
% }
% \scriptsize
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{c|cc||cc}
% \hline
% \multirow{2}{*}{Attack} & \TR & \METR & \multicolumn{2}{c}\METR  \\
%                         & \textbf{AUC} (\up)      & \textbf{AUC} (\up)  & \textbf{B acc} (\up) & \textbf{W acc} (\up) \\ 
% \hline
% None               & 1.000 (+0.0\%)     & 1.000 (+0.0\%) & 0.991   & 0.910    \\
% VAE~\cite{vae2018_attack}~$q=1$         & 0.999 (-0.1\%)     & 0.999 (-0.1\%) & 0.968   & 0.747     \\
% diff,~150 steps                & 0.952  (-4.8\%)   & \bf{0.999}(-0.1\%)  & 0.967    & 0.732      \\
% rotate 75               & \bf{0.959} (-4.1\%)    & 0.907 (-9.3\%) & 0.694   & 0.033         \\
% brightness 6.0          & 0.994 (-0.6\%)    & \bf{0.995} (-0.5\%) & 0.912   & 0.463     \\
% noise $\sigma=0.1$           & \bf{0.941}  (-5.9\%)   & 0.833 (-16.7\%) & 0.695   & 0.134       \\
% blur $r=4$                & 1.000  (-0.0\%)   & 1.000 (-0.0\%) & 0.979   & 0.805      \\
% crop 0.75               & \bf{0.911}  (-8.9\%)   & 0.807 (-19.3\%) & 0.668   & 0.020      \\
% JPEG 25                 & \bf{0.995} (-0.5\%)    & 0.992 (-0.8\%) & 0.953   & 0.719     \\
% \hline
% \end{tabular}
% \label{fig:all-att-default}
% \end{table}

\begin{figure}
\begin{floatrow}
\ffigbox{%
  \rule{3cm}{3cm}%
}{%
  \caption{A figure}%
}
\capbtabbox{%
  \begin{tabular}{cc} \hline
  Author & Title \\ \hline
  Knuth & The \TeX book \\
  Lamport & \LaTeX \\ \hline
  \end{tabular}
}{%
  \caption{A table}%
}
\end{floatrow}
\end{figure}

==> figures/table_tree_ring_metr.tex <==
% \begin{table}[h]
% \centering
% \caption{
%     Detection metrics for \TR and \METR. Note that \METR is almost as resilient to the attacks as \TR watermark.
% }
% \scriptsize
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{c|cc||cc}
% \hline
% \multirow{2}{*}{Attack} & \TR & \METR & \multicolumn{2}{c}\METR  \\
%                         & \textbf{AUC} (\up)      & \textbf{AUC} (\up)  & \textbf{B acc} (\up) & \textbf{W acc} (\up) \\ 
% \hline
% None               & 1.000 (+0.0\%)     & 1.000 (+0.0\%) & 0.991   & 0.910    \\
% VAE~\cite{vae2018_attack}~$q=1$         & 0.999 (-0.1\%)     & 0.999 (-0.1\%) & 0.968   & 0.747     \\
% diff,~150 steps                & 0.952  (-4.8\%)   & \bf{0.999}(-0.1\%)  & 0.967    & 0.732      \\
% rotate 75               & \bf{0.959} (-4.1\%)    & 0.907 (-9.3\%) & 0.694   & 0.033         \\
% brightness 6.0          & 0.994 (-0.6\%)    & \bf{0.995} (-0.5\%) & 0.912   & 0.463     \\
% noise $\sigma=0.1$           & \bf{0.941}  (-5.9\%)   & 0.833 (-16.7\%) & 0.695   & 0.134       \\
% blur $r=4$                & 1.000  (-0.0\%)   & 1.000 (-0.0\%) & 0.979   & 0.805      \\
% crop 0.75               & \bf{0.911}  (-8.9\%)   & 0.807 (-19.3\%) & 0.668   & 0.020      \\
% JPEG 25                 & \bf{0.995} (-0.5\%)    & 0.992 (-0.8\%) & 0.953   & 0.719     \\
% \hline
% \end{tabular}
% \label{fig:all-att-default}
% \end{table}

\begin{figure}
  \begin{minipage}[b]{.49\linewidth}
    \centering
    \captionof{table}{
    Detection metrics for \TR and \METR. \\
    Note that\\
    \METR is almost as resilient to the attacks \\
    as \TR watermark.
    }
    \scriptsize
    \renewcommand{\arraystretch}{1.5}
    \setlength{\tabcolsep}{1.8pt}
    \begin{tabular}{c|cc||cc}
    \hline
    \multirow{2}{*}{Attack} & \TR & \METR & \multicolumn{2}{c}\METR  \\
                            & \textbf{AUC} (\up)      & \textbf{AUC} (\up)  & \textbf{B acc} (\up) & \textbf{W acc} (\up) \\ 
    \hline
    None               & 1.000 (+0.0\%)     & 1.000 (+0.0\%) & 0.991   & 0.910    \\
    VAE~\cite{vae2018_attack}~$q=1$         & 0.999 (-0.1\%)     & 0.999 (-0.1\%) & 0.968   & 0.747     \\
    diff,~150 steps                & 0.952  (-4.8\%)   & \bf{0.999}(-0.1\%)  & 0.967    & 0.732      \\
    rotate 75               & \bf{0.959} (-4.1\%)    & 0.907 (-9.3\%) & 0.694   & 0.033         \\
    brightness 6.0          & 0.994 (-0.6\%)    & \bf{0.995} (-0.5\%) & 0.912   & 0.463     \\
    noise $\sigma=0.1$           & \bf{0.941}  (-5.9\%)   & 0.833 (-16.7\%) & 0.695   & 0.134       \\
    blur $r=4$                & 1.000  (-0.0\%)   & 1.000 (-0.0\%) & 0.979   & 0.805      \\
    crop 0.75               & \bf{0.911}  (-8.9\%)   & 0.807 (-19.3\%) & 0.668   & 0.020      \\
    JPEG 25                 & \bf{0.995} (-0.5\%)    & 0.992 (-0.8\%) & 0.953   & 0.719     \\
    \hline
    \end{tabular}
    \label{fig:all-att-default}
  \end{minipage}
  % \hfill
\begin{minipage}[b]{.49\linewidth}
    \centering
    \captionof{table}{
       Message decryption accuracy for \METRpp \\
       and its components: \METR and \Stablesig.\\
       Note that robustness of \METRpp \\
       is constrained by robustness of \METR or \Stablesig.
    }
    \scriptsize
    \renewcommand{\arraystretch}{1.5}
    \setlength{\tabcolsep}{1.5pt}
    \begin{tabular}{c|cc|cc|cc} 
    \hline
    \multirow{2}{*}{Attack} & \multicolumn{2}{c|}{METR: ft VAE} & \multicolumn{2}{c|}{Stable-Signature} & \multicolumn{2}{c}{METR++}  \\
                            &  Bit acc & Word acc                         & Bit acc & Word acc                    & Bit acc & Word acc          \\ 
    \hline
    None                                                        & 0.991   & \underline{0.914}   & 0.995   & 0.843                    & 0.995   & 0.772            \\
    VAE~~$q=1$                                                       & 0.970   & \underline{0.760}    & 0.490   & 0.000                      & 0.572   & 0.000         \\
    diff,~150 steps                                             & 0.966   & \underline{0.719}    & 0.477   & 0.000                  & 0.561   & 0.000          \\
    rot 75                                                        & 0.687   & \underline{0.029}    & 0.547   & 0.000                       & 0.572   & 0.000           \\
    bright 6.0                                                   & 0.909   & \underline{0.460}    & 0.904   & 0.264                      & 0.905   & 0.209           \\
    noise $\sigma=0.1$                                                & 0.694   & \underline{0.137}    & 0.539   & 0.000                       & 0.565   & 0.000          \\
    blur $r=4$                                                       & 0.981   & \underline{0.816}    & 0.419   & 0.000                      & 0.516   & 0.000         \\
    crop 0.75                                                        & 0.669   & 0.023    & 0.982   & \underline{0.569}                       & 0.928   & 0.013          \\
    JPEG 25                                                          & 0.941   & \underline{0.672}    & 0.769   & 0.000                       & 0.799   & 0.000         \\
    \hline
    \end{tabular}
    \label{fig:all-att-metrpp}
\end{minipage}
\end{figure}

==> sections/abstract.tex <==
% In recent years a lot of new methods for image generation were discovered, one of them is diffusion models ~\cite{diffusion_ddpm}. These models greatly improved on generation of high quality images, which might cause concerns about use of such images with illegal intentions in terms of policy on online platforms or even law. It becomes clear that it is necessary to recognize generated images and identify a person that generated it. All previous methods, that inject watermark in the process of generation suffer from low robustness to attacks or from inability to encrypt any or multiple unique messages, which can be used to assign individual keys to each user for large number of different users of API. We propose a solution that allows encryption of large amount of unique messages into images by improving Tree-Ring ~\cite{wen2023treering} watermarking method. We call our method \METR (Message Encoded Tree-Ring). We further improved \METR algorithm by introducing METR++, that allows to get as many unique messages as one might need. METR++ is a combination of our approach \METR and Stable Signature ~\cite{fernandez2023stable} watermark. We introduce \enquote{infinite} number of messages - extreme robustness tradeoff, the essence of which is in the robustness difference of METR and METR++. In the paper we will give clarity on \METR's capability of encryption of large amount of unique messages and will explain how we can use METR together with fine-tuned VAE decoders from Stable Signature to create METR++.

% In recent years a lot of new methods for image generation were discovered, one of them is diffusion models. These models greatly improved on generation of high quality images, which might cause concerns about use of such images with illegal intentions in terms of policy on online platforms or even law. It becomes clear that it is necessary to recognize generated images and identify a person that generated it. All previous methods, that inject watermark in the process of generation suffer from low robustness to attacks or from inability to encrypt any or multiple unique messages, which can be used to assign individual keys to each user for large number of different users of API. We propose a solution that allows encryption of large amount of unique messages into images by improving Tree-Ring watermarking method. We call our method METR (Message Encoded Tree-Ring). We further improved METR algorithm by introducing METR++, that allows to get as many unique messages as one might need. METR++ is a combination of our approach METR and Stable Signature watermark. We introduce "infinite" number of messages - extreme robustness tradeoff, the essence of which is in the robustness difference of METR and METR++. In the paper we will give clarity on METR's capability of encryption of large amount of unique messages and will explain how we can use METR together with fine-tuned VAE decoders from Stable Signature to create METR++.

Improvements in diffusion models have boosted the quality of image generation, which has led researchers, companies, and creators to focus on improving watermarking algorithms. This provision would make it possible to clearly identify the creators of generative art. The main challenges that modern watermarking algorithms face have to do with their ability to withstand attacks and encrypt many unique messages, such as user IDs. In this paper, we present METR: Message Enhanced Tree-Ring, which is an approach that aims to address these challenges. METR is built on the Tree-Ring watermarking algorithm, a technique that makes it possible to encode multiple distinct messages without compromising attack resilience or image quality. This ensures the suitability of this watermarking algorithm for any Diffusion Model. In order to surpass the limitations on the quantity of encoded messages, we propose METR++, an enhanced version of METR. This approach, while limited to the Latent Diffusion Model architecture, is designed to inject a virtually unlimited number of unique messages. We demonstrate its robustness to attacks and ability to encrypt many unique messages while preserving image quality, which makes METR and METR++ hold great potential for practical applications in real-world settings.
% Our code can be found at:~\href{https://github.com/deepvk/metr}{https://github.com/deepvk/metr}.

==> sections/citations.tex <==
\begin{document}

\end{document}
